Learning a Decentralized Multi-arm Motion Planner

We present a closed-loop multi-arm motion planner that is scalable and flexible with team size. Traditional multi-arm robot systems have relied on centralized motion planners, whose runtimes often scale exponentially with team size, and thus, fail to handle dynamic environments with open-loop control. In this paper, we tackle this problem with multi-agent reinforcement learning, where a decentralized policy is trained to control one robot arm in the multi-arm system to reach its target end-effector pose given observations of its workspace state and target end-effector pose. The policy is trained using Soft Actor-Critic with expert demonstrations from a sampling-based motion planning algorithm (i.e., BiRRT). By leveraging classical planning algorithms, we can improve the learning efficiency of the reinforcement learning algorithm while retaining the fast inference time of neural networks. The resulting policy scales sub-linearly and can be deployed on multi-arm systems with variable team sizes. Thanks to the closed-loop and decentralized formulation, our approach generalizes to 5-10 multi-arm systems and dynamic moving targets (>90% success rate for a 10-arm system), despite being trained on only 1-4 arm planning tasks with static targets. Code and data links can be found at https://multiarm.cs.columbia.edu.

==> text/backup/intro_v1.tex <==
\section{Introduction}
% 1 What is the problem you are solving? Why is the problem important?
% 2 Why is this problem challenging? Why do existing methods not work?
% 3 What is your key insight/idea? What is the trick that makes this work?
% 4 Overview of experiments. What are main conclusions of your experiments?
% 5 Summary of contributions

Many complex manipulation tasks can be decomposed into smaller sub-tasks which are efficiently distributed amongst multiple robotic arms in the same workspace.
% Give some examples.
A major challenge in designing motion planners for multi-arm systems is that the system's degrees of freedom (DoF) scales exponentially with the number of arms.
Prior works have focused on improving the run time of motion planners for systems with large DoFs by limiting the search space through discretization of the composite configuration space \cite{solovey2013drrt} \cite{shome2019drrtstar}.

Tasks for multi-arm systems are most naturally specified as a collection of target end effector poses, one for each arm in the system, and may vary with time.
Traditional multi-arm controllers \cite{mirrazavi2018unified} \todo{cite more} generally approach this problem in two parts.
First, an IK module finds collision free group goal joint configurations from the group target end effector poses.\todo{talk more about how IK in multi-arm works}
Next, a motion planning module computes collision free waypoints from the current group joint configurations to the group goal joint configuration specified by the IK module.
In a controlled assembly pipeline, motion plans only need to be computed once because the arms only perform repetitive tasks with low levels of uncertainty about its environments.


However, beyond the safe realms of such closed-room manufacturing and assembly applications, multi-arm systems could also engage in manipulation activities cooperatively with humans.
For instance, multiple robotic arms could aid in lifting heavy objects and handling large tools in construction sites, while the human worker guides the target motion of these arms with ease.
To find its place in such uncertain dynamic environments, multi-arm systems must have fast controllers, capable of planning and replanning its motion path within microseconds, a requirement which is unattainable for any solution with centralized controllers as the number of arms in the workspace increases.
\todo{TODO: Maybe not actually microseconds, but will replace with actual units in future revisions.}
Specifically, such centralized controllers must take into account every arm in the system in planning the motion for any single arm, regardless of whether a pair of arms could even reach each other, and therefore, collide with each other at all.
These ineffective use of computation power motivates a decentralized approach for multi-arm System controllers.

%
Decentralized controllers
\todo[inline]{TODO: History of designing decentralized controllers, multiagent systems, partial information, ... then talk about decentralized motion planners}
% TODO: challenges of design decentralized controllers
% Work on decentralized controllers for robotic arm systems


% Flexibility
An ideal characteristic of these multi-arm controller is flexibility with respect to the number of robot arms in the team.
As industrial demands change, team sizes may change as robotic arms are added or taken away, posing a challenge to centralized controllers that only work for a specific number of arms by treating the multi-arm system as one high degree-of-freedom robotic system.
Other applications that require flexibility are systems of mobile robots with arms that may move in and out of other robots' workspaces, and so must perform their task safely and efficiently regardless how many other robots are in its workspace.
These applications have computational complexity and flexibility requirements that are beyond the scope of existing methods.
\todo{Zhanpeng: previous sentence too aggressive, and need to talk first about what other works can achieve first before making this conclusion.}


While prior works addressed dual arm systems \cite{kurosu2017simultaneous} and a fixed-sized multi-arm systems \cite{mirrazavi2018unified},\todo{TODO: cite more works here} none has proposed a controller that works for all physically reasonable systems with any number of arms.
In this work, we present a scalable multi-arm controller by formulating multi-arm motion planning as a decentralized multi-agent learning problem.
\todo{break apart this previous sentence into more manageable chunks.}
Each arm observes the states of other arms within its workspace, and moves to reach its assigned target end effector pose while avoiding collisions with other arms.
The policy has a RNN base to account for the variable number of arms that could be present in each arms workspace.
Our approach is able to learn a multi-arm controller with low computational complexity with respect to the number of arms, as it contains no centralized component to act as the bottleneck of the system.


If arms are only rewarded for reaching their own end effector poses, arms do not learn to cooperate and allow other arms to reach their targets too.
To resolve these incentive issues, arms are only reward when all arms in the system have reached their target end effector poses, which makes an initially sparse reward setting even sparser.
We bypass the infeasibility of random exploration in this setting with expert demonstrations from BiRRT, which can be computed offline for a set of multi-arm motion planning tasks.
The expert trajectories are supplied to the Reinforcement Learning agent via the replay buffer when the agent fails to solve task, and withheld when the agent succeeds by itself.


\todo{TODO: talk about dynamic tasks}

==> text/backup/related_bk.tex <==
\section{Related Work}
% Single Arm Motion Planning
Sampling-based Motion Planners (SPMs) such as Rapidly-Exploring Random Trees (RRT) \citep{lavalle2006planning,karaman2011rrtstar} have long been the go-to solutions for generic motion planning.
%fueled excitement in the robotic applications due  to its probabilistically completeness and its run time over existing exact and complete combinatorial algorithms.
However, the runtime is exponential in the system's DoFs, which, for multi-robot systems such as multi-arm systems, is the sum of individual robots' DoF.
Another popular sampling-based planner is Probabilistic Road Maps (PRMs) \citep{kavraki1996prm}, which can achieve faster run times during execution than RRT, but generating sufficiently dense roadmaps for large DoF multi-robot systems is costly, and so, this approach is not flexible.

Many recent works have proposed learning-based approaches, which trade off a lengthy offline training stage for faster online execution.
\todo{Add \cite{jetchev2013fast} \href{https://link-springer-com.ezproxy.cul.columbia.edu/content/pdf/10.1007/s10514-012-9315-y.pdf}{paper} }
Prior learning-based works have improved the speed of SPMs by biasing the sampling distribution of new nodes \citep{ichter2017samplingdistributionrrt,qureshi2018deeply},
%
directly predicting the next node \citep{qureshi2019motion,qureshi2019motion2},
%
or reducing the search space through discretization \citep{solovey2013drrt,salzman2016multilinkdrrt,shome2019drrtstar}.
Many recent works have explored the application of reinforcement learning to motion planing \cite{zhang2018auto,pfeiffer2017perception,bency2018towards,faust2018prm}.
For example, Jurgenson et al. \citep{jurgenson2019rlmotionplanning} combined Deep Deterministic Policy Gradient \citep{lillicrap2015continuous} with expert demonstrations from RRT* for planar motion planning of a 4 DoF robot arm.
However, as these approaches do not explicitly account for multiple robots, they can only operate in a centralized fashion, and therefore is not scalable.
Though Berg et al. \citep{berg2005prioritizedmultirobot} explicitly account for multi-robot systems, their prioritized planning approach relied on \citep{berg2005roadmapdynamic} for motion planning which is open-loop, requires a lengthy computation of roadmaps for each specific workspace, and is still centralized.


Multi-arm motion planing problem has been studied in applications such as pick and place \cite{shome2019anytime} and table top rearrangement \cite{shome2018tabletop}.
Mirrazavi et al. \citep{mirrazavi2018unified} proposed a fast closed-loop multiarm controller capable of replanning at 500Hz for dual arm systems, but rely on a centralized Inverse Kinematics (IK) solver, whose constraints must be learnt from scratch if arms are added to, removed from, or moved around the workspace.
Most of these approaches also suffer from poor scalability because they have centralized components which may act as bottle necks in the system.


In order to achieve proper scalability, motion planners must be fully decentralized, where each robot solves a local optimization problem to reach its target configuration.
Non-Holonomic Optimal Reciprocal Collision Avoidance (NH-ORCA) \cite{alonso2013optimal} is a popular approach for distributed collision avoidance multi-robot planning, but is sensitive to hyper-parameters.
GA3C-CADRL \cite{everett2018ga3ccadrl} is a RL approach that uses an LSTM module to extract a fixed sized embedding from a variable number of other agents' observations, sorted by decreasing distance from the current agent.
% \cite{long2017towards} also decentralized motion plannig for planar robots https://arxiv.org/pdf/1709.10082.pdf
\cite{semnani2020multi} built on top of \cite{everett2018ga3ccadrl} with a hybrid deep RL and Force-based Motion Planning approach, which eliminated the need for a pretrained behaviour clone policy.
However, these approaches were applied to single-linked Clearpath Jackal ground robots in 2D and 3D configuration spaces, whereas our approach deals with tightly coupled multi-arm systems of 6 DoF UR5s.

% \cite{faust2018prm} combined PRMs with RL for mobile robot navigation, where PRM is used for long range planning and RL is used for low level control to satisfy task constraints and unmodelled environment dynamics, but does not explicitly account for the presence of other dynamic robots acting in the same environment.



% \textbf{Other works to read and include}:
% \begin{itemize}
%     \item \cite{ichter2017samplingdistributionrrt}: How is this different from  \citeauthor{qureshi2019motion}?
%     \item https://ipvs.informatik.uni-stuttgart.de/mlr/papers/13-jetchev-AuRo.pdf
%     \item https://www.cs.colorado.edu/~mozer/Teaching/Computational%20Modeling%20Prelim/Otte.pdf
%     \item https://ieeexplore-ieee-org.ezproxy.cul.columbia.edu/abstract/document/8809005
% \end{itemize}
